Striking a Balance: Reader Takeaways and Preferences when Integrating Text and Charts

While visualizations are an effective way to represent insights about information, they rarely stand alone. When designing a visualization, text is often added to provide additional context and guidance for the reader. However, there is little experimental evidence to guide designers as to what is the right amount of text to show within a chart, what its qualitative properties should be, and where it should be placed. Prior work also shows variation in personal preferences for charts versus textual representations. In this paper, we explore several research questions about the relative value of textual components of visualizations. 302 participants ranked univariate line charts containing varying amounts of text, ranging from no text (except for the axes) to a written paragraph with no visuals. Participants also described what information they could take away from line charts containing text with varying semantic content. We find that heavily annotated charts were not penalized. In fact, participants preferred the charts with the largest number of textual annotations over charts with fewer annotations or text alone. We also find effects of semantic content. For instance, the text that describes statistical or relational components of a chart leads to more takeaways referring to statistics or relational comparisons than text describing elemental or encoded components. Finally, we find different effects for the semantic levels based on the placement of the text on the chart; some kinds of information are best placed in the title, while others should be placed closer to the data. We compile these results into four chart design guidelines and discuss future implications for the combination of text and charts.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> original-submission/original00-abstract.tex <==
\abstract{ 
While visualizations are an effective way to represent insights about information, they rarely stand alone. When designing a visualization, text is often added to provide additional context and guidance for the reader. However, there is little experimental evidence to guide designers as to what is the right amount of text to show within a chart, what its qualitative properties should be, and where it should be placed.  Prior work also shows variation in personal preferences for charts versus textual representations. In this paper, we explore several research questions about the relative value of textual components of visualizations. 302 participants ranked univariate line charts containing varying amounts of text, ranging from no text (except for the axes) to a written paragraph with no visuals. Participants also described what information they could take away from line charts with text at varying levels of semantic content. We find that heavily annotated charts were not penalized; in fact, participants preferred the charts with the largest number of textual annotations over charts with fewer annotations or text alone.  We also find effects of semantic level; for instance, the text that describes perceptual or cognitive aspects of a chart leads to more takeaways than text describing statistical or relational components. Finally, we found different effects for the semantic levels based on the placement of the text on the chart; some kinds of information are best placed in the title, while others should be placed closer to the data. These results have important implications for chart design guidelines.

}

%We hypothesize that individuals' preferences for visual versus textual information vary, and likely so do their preferences with respect to the combination of the two. Furthermore, the content of textual components of charts ranges from describing low-level visual features to providing high-level takeaways on key insights.  
%There is a lack of empirical evidence on what types of text and its amount readers find useful to better understand the information presented to them.


%We examined how the presence and content of these varying semantic levels affect readers' takeaways. Findings from the study provide a better understanding of how readers integrate information when text and charts are paired together.

==> original-submission/original01-introduction.tex <==
\firstsection{Introduction}


Information visualization is usually defined as ``the transformation of data to visual representations'' \cite{ieeevis} or ``visual representations of datasets designed to help people carry out tasks more effectively.'' \cite{munzner2014visualization}. In research, visualization is often contrasted with alternative forms of presentation such as tabular or written descriptions.  However, in reality, most charts are displayed with accompanying text in the form of titles, annotations, and captions. Authors include text with charts to convey the core message of the data, draw readers' attention to specific parts of the chart, and provide explanations that readers may be unlikely to identify on their own~\cite{kosara2013storytelling}.  Appropriate text can provide additional context, potentially increasing the aesthetic appeal of a chart~\cite{segel2010narrative}.

Textual descriptions have been shown to be compellingly influential over the visual components of charts;  recent research has shown that the way a title is written can be the influencing factor on how a visualization is interpreted \cite{kong2018frames}, and that the textual component can be the most memorable part of a visualization in a memory task \cite{borkin2015beyond}.


Although some recent research has acknowledged the important role that textual context plays in visualizations, there is currently little scientific understanding of the best qualities, quantities, and positions of textual content within charts and graphs. On the contrary, studies of information visualizations often omit a text-only option when comparing charts \cite{stokesgive}, despite evidence that some people prefer text over charts, at least in certain circumstances \cite{hearst2019would}.

The goal of this paper is to add to our understanding of the role of text in visualizations and to help in the creation of guidelines for both designers and automated systems.  We examine questions of how much text people find helpful on a chart before it feels cluttered, what kind of text is useful to show in terms of the quality or semantics of that text, and how its placement affects both the chart reader's understanding of the underlying data and their preferences for how that information is presented.

Text often is present at different semantic levels, ranging from descriptions of the overall data, to specific visual features, to additional context to support framing the chart \cite{lundgard2021accessible}. It is not currently known which semantic level of text is best shown in the title, versus in an annotation close beside a line chart, or if it is better to show several annotations from the same level in all chart positions or to show one annotation from each of these levels in different positions in a chart.  It is not known how much is too much text, or if  charts can stand alone with almost no annotation.  

This paper describes empirical studies whose goals are to answer some of these questions. By
choosing a subset of a large design space, we try to answer how to find the sweet spot between under- and over-texting for relatively simple visualizations. Even these simple visualizations offer a useful and nuanced examination of the rich space encompassing textual and visual communication.





%Text helps add additional context, guidance, and directive to imagery such as illustrations and charts.~\cite{carney:2002,mayer_2020}. Readers often integrate text and pictorial information to develop a coherent mental representation of the information presented to them~\cite{bransford:1972}. Comprehending both the visual depiction of what is important in the imagery, along with suitable support from the accompanying text, could further enhance the reader’s understanding of the meaning of that representation. This overall understanding of the representation is the product of the interaction between the chart and imagery, along with the reader's knowledge from both prior and current that they discover as the reading progresses.

%Visualizations are relevant in the reading comprehension process because they help understand data more naturally. Many content sources,such as scientific papers and news websites, present the information using charts, diagrams, or tables that complement the text to improve understanding of concepts and ideas~\cite{ren:2017}. There has been a prevalence of text accompanying charts ranging from annotations, captions, to data-driven storytelling. Authors include text with charts to convey the core message of the data, draw readers' attention to specific parts of the chart, and provide explanations that readers may be unlikely to identify on their own~\cite{kosara2013storytelling}.  Furthermore, appropriate text can provide additional context, potentially facilitate the memorability of a chart and increase the aesthetic appeal of a chart~\cite{segel2010narrative}.

%Wolf~\cite{wolf2008proust} states that reading fluency is an important skill as it provides the extra time for the brain to infer, understand, predict, and interpret the meaning of the information when processing words. When text is used effectively with visuals, we get a preview of what lies ahead as we read, making it easier to understand what follows. As we continue to explore the role of text with charts in effective takeaways and reading comprehension, it is important to consider whether the juxtaposition of text with imagery interrupts the flow of reading or aids in further understanding. As we see an increase in the presence of charts and text coexisting together, we need to better understand how the semantics of text and its placement affect the chart reader's understanding of the data and their preferences for how that information is presented to them.

%However, it is not yet well understood how readers integrate text and charts during their takeaways, their preferences for how much text should be present with these charts, and the types of text that are most helpful when describing insights shown in the charts. Similar to the deliberate and thoughtful placement of marks with color and size encodings, it is important to carefully consider the construction of language based on its intended purpose in communicating aspects of the chart to the reader. While there is a definite utility of text to help add additional semantics to the data, when should an author include information and how much text is needed to clearly communicate the key message? Text often is present at different levels of semantics, ranging from titles that describe the overall data seen in the chart, annotations that describe specific visual features, and narrative text that provides additional context to support framing the key takeaway. Which of these semantic levels are most useful to a reader, and is there an appropriate amount of text that readers find useful and prefer to be included? In other words, when authoring charts, how does one avoid the pitfall of under- and over-texting?


% \subsection{Research Questions}
% \label{section:rq}
%  Previous research has shown that text is useful when emphasizing the same information as in the accompanying visualization~\cite{kim2021towards} and understanding the semantic content conveyed by it~\cite{lundgard2021accessible}. However, in this work, we wanted to better understand how readers integrate text with charts based on the amount of text and their various semantic levels, namely: (1) enumerating visualization construction properties (e.g., marks and encodings); (2) reporting statistical concepts and relations (e.g., extrema and correlations); (3) identifying perceptual and cognitive phenomena (e.g., complex trends and patterns); and (4) elucidating domain-specific insights (e.g., social and political context). Towards this goal, we ran a set of studies on univariate line charts to explore the following research questions: 

%\marti{These research questions now appear in 3 places in the text: here, in the Study design, and the results.  perhaps we should omit them from here.}
% \arvind{I think we could either cut this subsection altogether, or combine/condense it with the 4th/5th paragraphs of the intro which pose the space of questions. I personally prefer cutting this subsection and leaving the intro broad.}

% \begin{itemize}

% \item \textbf{RQ1}: What are readers' preferences when viewing charts with different amounts and semantic levels of text? How do these preferences vary based on readers' overall preferences for textual or visual communication?

% \item \textbf{RQ2}: How do the different semantic levels of text affect the type of information included in readers' takeaways? Further, when do readers include information in their takeaways that are not found either in the chart or the text?

% \item \textbf{RQ3}: How does text placement affect how readers integrate the text with the charts?

% \item \textbf{RQ4}: Which semantic levels of text do readers rely on when they come up with takeaways? 

% \end{itemize} 




%This paper explores the effects of text progression and the various semantic levels on readers' preferences and takeaways. Specifically, the contributions of our paper are:

The contributions of this paper include:
\begin{tight_itemize}
\item  Empirical studies with 302 participants on nine examples of univariate line charts with varied amounts and types of annotations to better understand user preferences and takeaways from those charts.
\item Results showing that participants prefer a combination of textual and visual communication over a single presentation style.
\item Results showing  that the choice of semantic content and placement of this semantic content as textual expression in a chart can influence what the participants take away from the chart.
\item A set of guidelines for where to place text on charts and what type of content to express.  
\end{tight_itemize}

The remainder of the paper is organized as related work (\S \ref{section:rw}),   experiment design and stimuli (\S \ref{section:study}), results of the experiment (\S \ref{section:results}), a discussion of the results (\S\ref{section:discussion}),  limitations and future work (\S \ref{section:lfw}), and conclusions (\S\ref{section:conclusions}).



% Previous research has shown that text is useful when emphasizing the same information as in the accompanying visualization~\cite{kim2021towards} and understanding the semantic content conveyed by it~\cite{lundgard2021accessible}. However, in this work, we wanted to better understand how readers integrate text with charts based on the amount of text and their various semantic levels, namely: (1) enumerating visualization construction properties (e.g., marks and encodings); (2) reporting statistical concepts and relations (e.g., extrema and correlations); (3) identifying perceptual and cognitive phenomena (e.g., complex trends and patterns); and (4) elucidating domain-specific insights (e.g., social and political context). Towards this goal, to explore the following research questions: 


\maketitle



==> original-submission/original02-related-work.tex <==
\section{Related Work}
\label{section:rw}

Our work exploring how readers integrate text with charts builds on guidelines and empirical work on composing text and visualizations, as well as considerations from systems and applications of these two modalities to visual analysis and data storytelling.

\subsection{Existing Guidelines and Empirical Results}

Stokes and Hearst advocate for text to be considered co-equal to visualization, calling for researchers to devote attention to concerns of readability and integration between these two modalities~\cite{stokesgive}. 
In this spirit, there is a growing body of work that explores the role that text plays in visual analysis and its importance for conveying the key message to the reader.

For instance, through eye-tracking studies, Borkin et al.~\cite{borkin2015beyond} find that participants fixated on and were more likely to recall the textual content of and around visualizations (including titles, labels, paragraphs, etc.).
Kong et al.~\cite{kong2018frames,kong2019trust} evaluate how titles can impact the perceived message of a visualization to find that participants were more likely to recall information conveyed by slanted framings (e.g., emphasizing only part of a chart's message) than the chart's visuals.
Troublingly, participants would only flag the slanted framing if it was especially egregious (e.g., offering a contradictory message to the chart); more subtle framings escaped unnoticed despite shaping participants' takeaways.
In contrast to these results, Kim et al. find that readers are perhaps able to mediate misalignments between text and visualization \cite{kim2021towards}. 
Through crowdsourced studies, they find that when both the chart and text describe a high-prominence feature, readers treat the doubly emphasized high-prominence feature as the takeaway; but, when the text describes a low-prominence chart feature, readers rely on the chart and report a higher-prominence feature as the takeaway~\cite{kim2021towards}. 

Earlier work by Mayer in multimedia communication provided rigorous
empirical support for nine theory-based effects of how people learn
from the combination of words and images \cite{mayer2002multimedia}.  One of these is the ``multimedia effect'', which
is the hypothesis that people can learn more deeply from the combination of words and images together than either alone. Subsequent studies have shown that
text placed in spatial proximity to explanatory images can reduce
cognitive load \cite{holsanova2005tracing,holsanova2009reading,zhao2014eye}.  However, the prior work does not provide guidance on the type of choices examined in this work.

Text is a primary means for making visualizations accessible to people who are blind or have low vision (BLV). 
The W3C Web Accessibility Initiative (WAI), visualization practitioners, and publishers of accessible media have produced a variety of guidelines for what these textual representations (referred to as alternative text or alt text) should seek to convey including the chart type, axes and labels, and summaries of the overall trends~\cite{w3c_wai_2019, cesal_writing_2020, benetech_making_nodate}.  
Building on these guidelines, Jung et al. survey and interview BLV people to find that, when available, alt text is often the only interface to the depicted data; thus, poor quality text can often increase inequities in information access~\cite{jung2021communicating}.
The researchers further recommend that alt text should be structured to aid readers in mentally reconstructing, grounding the textual representation in the underlying data rather than visualized elements to reduce readers' cognitive burden. 
These findings are corroborated by Portluri et al., who find that BLV users already understand and benefit from having access to concepts of spatiality and visual semantics (e.g., size, shape, location) of user interfaces~\cite{potluri_examining_2021}.

Most related to our work is a recent paper by Lundgard and Satyanarayan that begins to formalize the semantic content that textual descriptions of charts can convey~\cite{lundgard2021accessible}. 
They develop a conceptual model that spans four levels of semantic content: enumerating visualization construction properties (e.g., marks and encodings); reporting statistical concepts and relations (e.g., extrema and correlations); identifying perceptual and cognitive phenomena (e.g., complex trends and patterns); and elucidating domain-specific insights (e.g., social and political context). 
In studies with sighted and blind participants, the researchers find that these reader groups differ significantly on which semantic content they ranked as most useful: while sighted participants generally preferred descriptions that offered high-level explanations and domain-specific context, blind readers poorly ranked these captions and instead favored either mid-level descriptions of statistical features or perceptual trends, or expressed bi-modal preferences for low-level details about the chart's construction. 
Inspired by this work, we apply Lundgard and Satyanarayan's four-level model of text semantics to further understand how the presence or absence of these levels of text and their placement in line charts affect sighted readers' preferences and takeaways. 



\subsection{Visualization + Text for Analysis and Storytelling}

Researchers are increasingly exploring how to leverage the unique affordances of natural language text during visual analysis~\cite{srinivasan2017natural}.
For instance, systems like Articulate~\cite{sun2010articulate}, DataTone~\cite{gao2015datatone}, and Eviza~\cite{setlur2016eviza} demonstrate that the familiarity of natural language statements can provide a shallower on-ramp to visual analysis, and the ambiguity of these statements can be used to more rapidly suggest candidate visualizations. 
These systems, however, consider each statement in isolation and subsequent work explores how pragmatics~\cite{hoque2017applying} and question-answering pipelines~\cite{dhamdhere2017analyza, kim2020answering} can aid in a more conversational interaction model.
In this context, the work most relevant to our contribution is a pair of studies exploring visual analysis via chatbot interfaces~\cite{hearst2019would, setlur2022gricean}\,---\,these studies demonstrate significant differences in whether participants prefer analysis results to be conveyed via text (or speech), visualization, or both.
These results provide inspiration for the research questions we pose in this paper, namely around preferences for how text and visualization modalities should be composed together. 




Besides serving as input or output for visual analysis,  systems have begun to incorporate natural language-generated text along with their visualization responses to help describe key insights to the user.
For example, a variety of research systems~\cite{mittal1998describing, srinivasan2018augmenting, kanthara2022chart, chen2020figure, qian2021generating} and popular tools such as Tableau's Summary Card~\cite{tableausummary}, Narrative Science~\cite{ns}, and Power BI~\cite{powerbi} produce natural language captions that summarize statistics and trends depicted by the chart.


Data storytelling weaves data, textual narratives, and visuals together for sharing and communicating insights that are more memorable, persuasive, and engaging than statistics alone~\cite{segel2010narrative,kosara2013storytelling, lee2015more}. With the growing recognition of using both text and charts for data storytelling, there is an added challenge of helping readers synthesize information from both text and charts in documents, especially when they are spatially separated.  Systems like Kori~\cite{latif2019authoring, latif2021kori} and VizFlow~\cite{sultanum2021leveraging} provide explicit linking strategies between the two modalities following design patterns that have emerged for data storytelling and narrative sequencing and rhetoric~\cite{hullman2013deeper, hullman2011visualization}.
While these systems demonstrate the utility of designing text and charts in concert, it is still unclear how to balance between the two modalities (e.g., is too much or too little text still useful?). Our work probes these research questions and provides design implications for future systems for jointly authoring text and visualization. 




%%%%% 
% OLD TEXT BELOW:
%%%%%



% Data visualizations are often organized in sequences to convey data stories where visualization viewers examine not only individual charts but also the relationships between them~\cite{kim2017graphscape}. As part of constructing narrative structures, causal coherence is found to be a significant discourse factor for describing sequencing and continuations in the narratives~\cite{das:2018,dasgupta2018automatic}. Causal relations can be specified in various forms, such as marking a cue phrase indicating the causal relationship, explicitly or implicitly stating both the cause and the effect)~\cite{blanco2008causal}. While the expression of causal relations in text can be very different, automatically detecting causal mechanisms from text could be used to summarize key takeaways more quickly~\cite{nazaruka2019identification}. Coherent narratives contain a set of related text discussing a particular topic with information related to different subtopics. Text Tiling was a technique that explored the division of expository text into multi-paragraph sub-topical segments making use of patterns of lexical co-occurrence and distribution within texts~\cite{Hearst1997}. While text can help build a narrative for the reader to take away key insights, our work further explores how viewers integrate text with charts.

% %Rhetorical/narrative/visualization devices
% Although visualizations are often seen as neutral and objective, various design choices for data visualization together with the journalistic organizational practices may add the potential framing effect to the data stories~\cite{hullman2011visualization}. Kennedy et al. examined the conventions that shape data visualization for visual communication, centered on the rhetorics of objectivity, transparency, and facticity~\cite{kennedy2016work} Mahyar et al. argued for viewing engagement at multiple levels and proposed a preliminary taxonomy for evaluating user engagement~\cite{mahyar2015towards}. % The use of schematic figures as graphical cues, such as freeform annotations and overlays on visually salient features in charts and their influence on comprehension and verbal descriptions, have been the subject of research in diagrammatic communication~\cite{kong09,kong2012graphical}. We draw inspiration from this body of work to further explore how the amount of text, its placement in the chart, and its semantic level frame the rhetoric of the key message communicated to the viewer.




\begin{figure*}[t!]
 \centering
 \includegraphics[width=\linewidth]{figures/stimuli_design1.pdf}
 \caption{How stimuli are created: Annotations are written and placed based on the components of the chart, which are identified as visually salient using the method from  \cite{kim2021towards}. The initial chart is shown in (a). In (b), red indicates the most visually salient feature, green the second, and blue the third. In (c) authors created potential annotations for each salient region at each level L2-L4. L1 cannot refer to a part of the chart identified as salient, but as shown in (d), it can refer to different areas of the chart (axis, trend, and title). A `trend' placement refers to an annotation which describes the line as a whole. L2-4 can each be placed in the same positions, as shown in (e); they can be expressed in a point, a trend, or as the title. In step (f), an expert designer adjusts the fine details to produce a chart with a realistic layout.  }
 \label{fig:stimuli_creation}
\end{figure*}


==> original-submission/original03-evaluation.tex <==



\section{Study}
\label{section:study}

In this study, we explore three primary research questions and their corresponding hypotheses: 

\noindent \textbf{RQ1}: What are readers' preferences when viewing charts with different amounts of text? To investigate this question, participants ranked charts with varying amounts of text, including an all-text paragraph. We hypothesized the following: 
\begin{tight_itemize}
\item \textbf{H1a}: Readers with an overall preference for visual information will prefer charts with annotations compared to the all text version.
\item \textbf{H1b}: Readers with an overall preference for textual information will prefer the all text variant compared to charts with little or no text.
\item \textbf{H1c}: Readers with an overall preference for visual information will prefer charts with fewer annotations.
\item \textbf{H1d}: Readers with an overall preference for textual information will prefer charts with a greater number of annotations.

\end{tight_itemize}

In investigating these hypotheses, we created two sets of ranking stimuli. The first encompassed the `extremes' within the range from text to visual. This included a chart with no text (except axes) to a text paragraph with no chart (see Figure~\ref{fig:teaser}). The second set of stimuli examined more fine-grained differences, ranging from a chart with only a title to a chart with a title and two annotations (see Figure \ref{fig:ranking_sets}).

\medskip

\noindent \textbf{RQ2}: How do the different semantic levels of text affect the type of information included in readers' takeaways? Further, when do readers include information in their takeaways that are not found either in the chart or the text? Which semantic levels of text do readers rely on when they form their takeaways? 

Hypotheses were as follows:
\begin{tight_itemize}
\item \textbf{H2a}: Readers' takeaways will be more likely to contain a given semantic level if the text accompanying the chart also contains that semantic level. This will be true for all semantic levels.

\item \textbf{H2b}: Readers will be more likely to include information in their takeaways that are not found in the chart or text when L1 is present in the chart.
\item \textbf{H2c}: Readers will self-report as relying \emph{less on text} and \emph{more on the chart} when the text contains L1.
\item \textbf{H2d}: Readers' takeaways will rely more on text when the text contains L4.
\item \textbf{H2e}: Readers with an overall preference for textual information will rely more on text within a chart. 
\end{tight_itemize}

\noindent \textbf{RQ3}: How does the placement of text affect how the reader integrates the text with the chart? Our hypothesis was:
\begin{tight_itemize}
\item \textbf{H3}: Readers' takeaways will be most likely to contain a given semantic level if the text containing that semantic level is positioned on the top left than text positioned on the bottom right.
\end{tight_itemize}


\noindent
To investigate research questions 2 and 3, participants were asked to inspect a chart with varying annotations at varying semantic levels, and then provide up to three takeaways.  

%We hypothesized the following, ordered by the research questions in Section \ref{section:rq}.



To test these hypotheses, we designed the stimuli to systematically vary the content and location of the textual annotations. Since these hypotheses, for the most part, do not concern the quantity of text, the charts displayed in this section contained only a title or a title and a single annotation. See Section \ref{section:stimuli} for further information on development of the stimuli. 
%This section expanded the work in \cite{kim2021towards} to examine on- annotations and titles.

\begin{figure*}[t]
 \centering
 \includegraphics[width=\linewidth]{figures/ranking_sets.pdf}
 \caption{Example stimuli for ranking set B (fine-grained comparisons). An example of ranking set A (`extremes') appears in Figure~\ref{fig:teaser}. 
 }
 \label{fig:ranking_sets}
\end{figure*}

\subsection{Participants}

Based on a power analysis with G*Power \cite{faul2007g} on a logistic regression with an odds ratio of 1.5 and a desired power of 0.8, the proper sample size (post exclusions) is 297, with an alpha level of 0.05. This also accommodates the sample size recommended from an additional analysis on a Friedman's test.


We recruited 512 participants from Amazon Mechanical Turk. In order to qualify for the study, participants were required to be located in the United States and to have a 95\% acceptance rate on previous tasks. We also required that they be fluent in English and complete the survey on a desktop or laptop device. We compensated participants at a rate of \$15 per hour. This resulted in a \$3.50 compensation for a 14 minute survey, which was raised to \$4.00 based on a longer survey time than estimated. We employed comprehension checks in the first block of the survey. If they missed both comprehension questions, their survey ended. An attention check was employed prior to the section eliciting takeaways. Participants completed a filter task, as shown in Figure \ref{fig:survey_flow}. If they selected any incorrect options, they were compensated the full amount but were excluded from the analysis. We also implemented an attention check about halfway through the survey to ensure that workers were paying attention. Those who failed the attention check were also compensated the full amount but excluded from analysis. Participants were also not permitted to take the survey multiple times. 

After excluding these participants as well as any who provided extremely low-quality responses (e.g., takeaways that were either unintelligible or off-topic), we ended up with 302 participants. On average, participants were 35-44 and most had completed a 4-year degree. On a scale from 1 indicating an overall preference for textual communication and 6 indicating an overall preference for visual communication, participants had an average score of 4.06 across the measures used.

\subsection{Stimuli}
\label{section:stimuli}
All stimuli used in this study were univariate line charts, adapted from Kim et al. \cite{kim2021towards}. We considered univariate line charts for our work because they are among the most common basic charts and are easily parameterizable, making them useful to explore our hypotheses. A subset of nine charts from the original paper was generated. To keep the overall design space tractable, we generated a set of synthetic line charts containing one positive trend, while maintaining realistic global shapes. This chosen shape introduced sufficient variation in the stimuli, while maintaining enough blank space on the chart in which to situate textual and visual annotations. We also added aesthetic design updates to the charts, such as providing lightened gridlines and axes ticks. The data line itself was also darkened. These aesthetic changes were completed to align the stimuli to more ecologically valid designs, with advice and design style provided by a visualization designer. To provide context to the charts, we labeled the x-axis with time unit values implying that the chart represents a time series. Specifically, we selected the start and end of the x-axis from the set of years {1900, 1910, 1920,..., 2020}. To label the y-axis, we randomly chose a set of domains for the y-axis and its value range from the MassVis dataset \cite{borkin:2013}.


\subsubsection{Annotation content}

We wrote four possible textual annotations to be added to each chart. Each of the four annotations per chart contained information from one of the semantic levels outlined by Lundgard \& Satyanarayan \cite{lundgard2021accessible} as described below:

\begin{tight_itemize}
\item \textbf{Semantic Level 1 (L1)}: The first level consisted of elemental or encoded aspects of the chart, such as the overall topic or a description of the content of an axis. For example, in Figure \ref{fig:teaser}, \textit{``President approval rating over 5 years (2015-2020).''}
\item \textbf{Semantic Level 2 (L2)}: The second level consisted of statistical or relational components, such as a comparison between two points or identification of extrema. For example, in Figure \ref{fig:teaser}, \textit{``Maximum''}.
\item \textbf{Semantic Level 3 (L3)}: The third level described perceptual or cognitive aspects, such as an overall pattern or changes in trend. For example, in Figure \ref{fig:teaser}, \textit{``Steep fall slows to a steady decrease.''}
\item \textbf{Semantic Level 4 (L4)}: The fourth provided external context to the chart, such as fictional past events which affected the topic depicted. These were created with reference to Wikipedia articles pertaining to the topic of each chart to create plausible commentary \cite{wikipedia2004wikipedia}. For example, in Figure \ref{fig:teaser}, \textit{``President starts popular initiatives against child hunger''}. Sighted readers most preferred this level in \cite{lundgard2021accessible} and visualization designers often include it as a part of best practices \cite{knaflic_2017}.
\end{tight_itemize}

These annotations were written by one author in collaboration with another to ensure that the semantic content was consistent with the descriptions for each of the four semantic levels. Annotations were not computationally generated to maintain ecological validity in the stimuli themselves. Especially for L3 and L4, we wanted to ensure that the annotations reflected ``natural sounding" language, as the definitions of those levels rely in part on human perception and cognition.


The content for each of the annotations was written based on the visually salient features in the line charts, as shown in Figure \ref{fig:stimuli_creation}. Identification of these visually salient features was computed using crowdsourced data from Kim et al. \cite{kim2021towards}. Saliency mapping takes into consideration mouse input information for bounding boxes that users drew around features that they identified as the top three visually prominent features in the line charts. We aggregated all of the feature bounding boxes by projecting each box onto the x-axis to form a 1D interval, weighting each interval inversely proportional to the ranking provided by the crowdsourced data. We then multiplied the weight assigned to each interval by a Gaussian factor centered at the interval and with standard deviation set to half the width of the interval. Summing all of the Gaussian weighted intervals, we obtained the top three visually salient regions for each line chart stimulus.

The visual salience of each semantic level was counterbalanced between the nine selected data shapes, such that each semantic level had the same average visual salience across the stimuli set. However, L1 did not refer to any particular point or area within the data, and so could not be mapped to visually salient features. This counterbalancing was only completed for L2 - L4. More detail about this process is shown in Figure \ref{fig:stimuli_creation}.



\subsubsection{Annotation appearance and position}
Annotations were added to the line charts with the aforementioned visually salient features based on feedback from an expert data visualization designer. The progress from a blank chart through the full set of possible annotations can be seen in Figure \ref{fig:stimuli_creation}. Design practices include standard conventions \cite{few2004show, knaflic2015storytelling, tufte1985visual, wong2010wall} to prioritize focus on the line. The line color was selected to blend in with the blue used elsewhere in the survey instrument without creating a visual artifact for users with astigmatism \cite{locke_2021}. All text met at least AA guidelines under WCAG 2.0 testing. The placement of the annotations was guided by the following design guidelines.

\begin{tight_itemize}
\item \textbf{Legibility}: Avoid adding annotations too close to one another or overlapping \cite{kirk2016data,  wong2010wall}.
\item \textbf{Visual language}: Add banding to depict time ranges, show arrows for trends, and dots for point-in-time references.
\item \textbf{Spatial agreement}: The label should follow the pattern of the data and be as close to the referent as possible. 
\end{tight_itemize}

The overall placement of the annotations was counterbalanced across the set and between the four semantic levels. For example, each semantic level was positioned in the title or subtitle position three times. These stimuli and their annotations underwent several rounds of iteration through the processes in Figure \ref{fig:stimuli_creation}. 



For each chart in the stimuli set, we also included an all-text version, as advocated for by Stokes \& Hearst \cite{stokesgive}. Three authors created textual descriptions of the chart, incorporating the additional information chosen to accompany the chart. These three versions were then discussed and synthesized into a single paragraph with feedback from all authors. From this paragraph, an additional chart was created to convey the same story as the all text paragraph, to preserve dynamic equivalence \cite{metzger_1999}. Here, we aimed to create parity between visual and textual, regardless of the amount of text required. These annotations were also created using the guidelines above. The full set of possible stimuli as well as their all-text descriptors can be found in the supplementary materials.



\subsection{Method}

\begin{figure*}[ht]
 \centering
 \includegraphics[width=\linewidth]{figures/survey_flow.pdf}
 \caption{Participants completed a survey with the six sections above: terminology introduction, individual viewing of stimuli, ranking of the full stimuli set, filter task, entering takeaways, graphical literacy, and demographics. Individual viewing and ranking were completed for both ranking sets.}
 \label{fig:survey_flow}
\end{figure*}

Participants completed a survey with five main sections. The full survey flow can be seen in Figure \ref{fig:survey_flow}. First, participants were introduced to the study and the terminology used throughout the survey. They were instructed in how to apply the terms \emph{axis}, \emph{visual}, and \emph{text}, with \emph{text} deconstructed into \emph{title} and \emph{annotation}. They were then asked to answer 1-2 questions to check for understanding of this knowledge and were provided with an illustration of the terminology after each question. Those who answered the first question correctly were not asked the second question. 



After this introduction, participants went on to complete the first set of ranking tasks. They were instructed: ``In the next section, you will rank two sets of images. During this section, keep in mind the following instructions. Rank the images in the order you would prefer to encounter or see them. You can rank by dragging and dropping the subsequent images into a rank.'' The ranking tasks within this survey were designed to elicit user preferences for the amount of text paired with a chart. Prior to completing the ranking, participants viewed each stimulus individually and answered a free-response question about the qualities of the information presentation which they liked and those which they disliked.

The stimuli for the first set of charts (Set A) consisted of four items: a chart with only axes labels and tick marks, a chart with a title and an on- annotation, a chart with a story or narrative about the data annotated, and a paragraph of entirely text which described the chart shown. In set A, we aimed to capture preferences for the ‘extremes’ between an (almost) entirely visual presentation of information and an entirely textual presentation. The second set of charts (Set B) consisted of three charts: one with only a title, one with a title and an on- annotation, and one with a title and two annotations. With this set, we examined a more detailed variation in the number of on- annotations, progressively increasing it within the set. Specific chart combinations within sets were also selected to best counterbalance between annotation position and content. 
%An illustration of the individual viewing and ranking task with example stimuli can be seen in Figure \ref{fig:ranking_task}. 

%\begin{figure}[h]
% \centering
% \includegraphics[width=0.9\linewidth]{figures/ranking_task.pdf}
% \caption{An illustration of the individual viewing (a) and ranking task with example stimuli (b). 
%\marti{I think this figure can be omitted for space considerations.} }
% \label{fig:ranking_task}
%\end{figure}
% if low on space, cut and move to appendix

Following the ranking task, participants went on to complete a filter task, which also provided them with some training on our definition of `takeaway'. In this task, participants were shown a chart and five example takeaways that could be drawn from the chart. Three of the five were true statements about the chart, while two were false. Participants were instructed to select those which were true. If the participant selected any options which were incorrect, their survey ended and they did not go on to the following sections.

If they selected all and only the correct takeaways, participants moved on to the takeaway section of the survey. In this section, participants were shown a chart and told that they would be asked to generate takeaways on the following page. They were also informed that they would not be able to go back and view the chart after moving on. They were allowed to spend as long as they felt necessary on this page and selected a button to indicate they were ready to move forward. Charts shown in this section contained either only a title or a title and a single on-chart annotation. This resulted in a set of ten possible combinations per data shape, considering the pairwise combinations of the four semantic levels. 
%A depiction of the possible combinations for a single data shape can be seen in Figure \ref{fig:teaser}. 
On the page following the image of the chart, participants were asked to provide their takeaways.
Takeaways were defined as ``a key fact, point, or idea to be remembered after viewing the chart.''
They were required to provide at least one but had the option to provide up to three takeaways.  They were also asked to rate ``Which aspect of the information did you rely on when listing your takeaways?'' on a scale from 1 (``entirely text'') to 5 (``entirely visual''). 

The fourth section of this survey was a subjective measure of graphical literacy \cite{garcia2016measuring}. Participants were asked to report how good they considered themselves to be at working with different chart types, such as line, bar, and pie charts. As part of this measure, they were also asked questions regarding their preference for textual or visual information, such as ``When reading books or newspapers, how helpful do you find charts that are part of a story?'' and ``To what extent do you believe in the saying `a picture is worth one thousand words'?''. We added an additional question to this section beyond the graphical literacy measure, ``To what extent do you believe in the saying, ‘Reading expands the mind'' which was reverse coded for preference for visual information.

Finally, participants completed the demographic section. Here, they reported their age range (e.g., 18-24), their current education level (e.g., ``Less than high school''), and their experience with charts and reading. This experience was captured through both the frequency (e.g., ``Every day'') as well as the context in which they engaged with the material (e.g., Government reports). For reading, we inquired about the frequency of both short-form reading (e.g., text messages, tweets) as well as long-form (e.g., books, magazines). 

\section{Results}
\label{section:results}

In this section, we provide results for research questions RQ1 -- RQ3.  Each research question is assessed in terms of a set of hypotheses as enumerated in Section~\ref{section:study}.
Analysis plans were preregistered on OSF.\footnote{\url{osf.io/vz976/?view\_only=178d12f1f53d4dfabaa39a3ceb0618cc}} 

\pheading{Visual vs. Textual Preferences.}
Hypotheses below compare participants with an overall preference for visual information (the \textsc{visual} group) and those with an overall preference for textual information (the \textsc{textual} group). To calculate a preference score for each participant, we summed up the Likert ratings for the questions included in the measure of graphical literacy \cite{garcia2016measuring} and questions regarding the frequency of reading text and viewing charts, included in the demographics section. Those in the `\textsc{visual} group were in the top 25\%
of the set of summed scores, and those in the \textsc{textual} group were in the bottom 25\%.


\subsection{RQ1: Preferences for Amount of Text}
RQ1 asks: what are readers' preferences when viewing charts with different amounts of text?


\pheading{Summary of Findings:} Overall, we found a strong preference for the charts with a greater number of annotations. For both sets ranked, the highest performing stimulus was the chart with the most annotations. While some participants did not like the clutter created by the annotations, they still ranked it above other  variants. They preferred \textit{receiving} the information and rated the no-text variant or title-only variant consistently lowest due to its lack of context and message. 


\begin{figure*}[t]
 \centering
 \includegraphics[width=0.9\linewidth]{figures/ranking_results.pdf}
 \caption{Ranking task results, shown for all participants as well as the \textsc{visual} and \textsc{textual} groups. Pairwise significance can be seen in Tables \ref{tab:rank_setA} and \ref{tab:rank_setB}. Lines within columns indicate statistically significant relative rankings (* = 0.05, ** = 0.01). \newline a) Ranking set A (`extremes'). b) Ranking set B (`fine-grained'). 
 }
 \label{fig:ranking_results}
\end{figure*}


\pheading{Details of Analysis:} To examine this question more closely, we completed Friedman's tests for the rank-order data. We performed post-hoc Nemenyi's tests to examine pairwise comparisons, shown in Tables \ref{tab:rank_setA} and \ref{tab:rank_setB}. Overall relative stimuli rankings can be seen in Figure \ref{fig:ranking_results}.

In both ranking tasks, the most heavily annotated charts were ranked highest overall.  In Ranking Set A, the chart with the story was highest ranked across participant types, while the next most annotated chart tied with the textual paragraph for second place for those people who prefer text.  The spare ``under-texted'' chart with minimal annotations ranked lowest across conditions -- participants least preferred the no-text version from Set A and the chart with only a title from Set B.  

%Participants preferred charts that we had thought may have been ``over-texting.'' They most liked the chart with the story from the `extremes' and the chart with two annotations and a title from the `fine-grained'. However, there was a strong dislike for charts that were ``under-texting', as participants least preferred the no-text version from the `extremes' and the chart with only a title from the `fine-grained'. 
%\arvind{This paragraph says we (the authors) considered charts to be over/under texting but I'm looking at earlier sections and although we use these terms, we seem to only do so loosely without a precise definition? Maybe I missed it, but otherwise I'm having trouble making sense of this paragraph summary of results.}
%\marti{This has bothered me as well; I want to rewrite this paragraph}

Hypotheses 1a and 1b below refer to the rankings of the `extremes', shown in Figure \ref{fig:teaser}, while 1c and 1d refer to the `fine-grained' rankings, shown in Figure \ref{fig:ranking_sets}. 
% text or textual?
% figure note - for each set, overall in the middle, broken out to text to the left and visual to the right.

% \noindent 
\subsubsection{H1a, b: Preferences Compared to All-Text}

\textbf{H1a:} \textit{Readers with an overall preference for visual information
will prefer charts with annotations compared to the all text version.} 
This hypothesis was \textbf{supported} ($\chi^2 = 151.15$, df = 3, $p < 0.01$). For the \textsc{visual} group, the chart with the most text received the highest average rating (1.37), while the all text version tied with no-text for the lowest rating (3.21).

\smallskip
% do i need the numbers here?
\noindent 
\textbf{H1b:} \textit{ Readers with an overall preference for textual information will prefer the all text variant compared to charts with little or no text.}
This hypothesis was \textbf{partially supported}. Overall, the average rankings for the stimuli differed ($\chi^2 = 50.962$, df = 3, $p < 0.01$). For the \textsc{textual} group, the all-text version (2.42) was tied for second place with the chart with a title and single annotation (2.41). Therefore, there was no difference between all-text and a chart with little text. However, the no-text chart was rated lowest (3.24). So, we find partial support for this hypothesis in comparison to the no-text.

 \noindent 
\textbf{H1c}: \textit{Readers with an overall preference for visual information will prefer charts with fewer annotations.}
This hypothesis was \textbf{not supported}, though the average rankings of stimuli did differ ($\chi^2 = 75.25$, df = 2, $p<0.01$). The \textsc{visual} group most preferred charts with the greater number of annotations, rather than those with fewer.

\smallskip
 \noindent 
\textbf{H1d}: \textit{Readers with an overall preference for textual information will prefer charts with a greater number of annotations.}
This hypothesis was \textbf{supported}, as results were similar to the \textsc{visual} group ($\chi^2 = 21.24$, df = 2, $p<0.01$). The \textsc{textual} group also most preferred charts with the greater number of annotations, rather than those with fewer.


% \marti{This is new; please comment on this subsection.  I plan to add some more similar analysis unless people think it is not rigorous or interesting enough.}
 %\arvind{I like where this subsection is going. The points its currently making across the two paragraphs feel a little duplicative but that's probs because this is still a WIP. I'd be curious if participants made comparisons between the options, or if there was pushback about some of them (e.g., people not liking the all text option or annotations because it's doing the ``interpretation'' for them, etc.)? My other comment is that the results being reported in this section still rely heavily on counting, so maybe we don't want to distinguish with quant/qual headings and just have an overall subsection of results? (Unless of course we begin to report out the free response answers more.) \marti{Good points; maybe we can remove qualityative/quant distinction and only focus on the outliers which is what I was mainly interested in.}}

%As noted in the overall results for RQ1, most participants in conditions A and B  preferred charts annotated with more text. The 63\% of participants who ranked the annotation-heavy story  highest in set A (Figure \ref{fig:teaser}(c)) frequently commented on the how the text added clarity and helped to explain the meaning of the chart, or commented favorably on the amount of detail that this  type contained.  Some wrote that they preferred this chart despite its looking crowded or cluttered.

Although most participants ranked the annotation-heavy chart in Ranking Set A highest,
this data also shows that a substantial minority\,---\,42, or 14\% of participants\,---\,ranked the all text option as their first choice for Set A.  Of these, 25 are identified by our analysis as text-preferred, 5 as visual preferred.  One author examined the comments participants made both when discussing the all text view and (optionally) the reason for their ranking.  The primary reasons given for preferring the textual paragraphs over the three charts were (repeat participants allowed): 
\begin{tight_itemize}
    \item General preference for text over charts (7),
    \item Text perceived as clearer, more understandable, and/or providing a better explanation (13),
    \item Text perceived as providing a better story or context, or more interesting (4),
    \item Text perceived as more precise,  concrete, or thorough (9).
\end{tight_itemize}
Interestingly, two participants stated that they preferred reading text and using their imagination to see the trends.  Of those classified as visual preference, two mentioned details, one mentioned clarity, and two did not address the issue.

A few (15) participants ranked the no-text chart highest.  The most common reasons given were simple / easy to understand (9), clean/lack of clutter (5), and allows the viewer to draw their own conclusions (4).  





%tables for pairwise comparison values - i hate tables in latex so if someone can make this look nicer, please do
\begin{table*}[t]

\def\arraystretch{1.5}
    \centering
    \begin{tabular}{ | m{0.12\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} |} 
      \cline{2-7}
      \multicolumn{1}{c|}{}
        & No-text, \newline Title+one & No-text, \newline  Story & No-text, Text & Title+one, \newline  Story & Title+one, Text &  Story, Text \\ 
      \hline
      Visual & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & p = 1 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 \\ 
      \hline
      Textual & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!5}p $<$ 0.05 & p = 1 & \cellcolor{blue!5}p $<$ 0.05 \\ 
      \hline
      All Participants & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 &\cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 \\ 
      \hline
    \end{tabular}
    \caption{Pairwise comparisons between preference groups for the 'extremes' ranking set (A). 
    }
    \label{tab:rank_setA}
\end{table*}

\begin{table}[h]
\def\arraystretch{1.5}
   \centering
    \begin{tabular}{ | m{0.2\linewidth} | m{0.2\linewidth} | m{0.2\linewidth} | m{0.2\linewidth} |} 
      
      \cline{2-4}
      \multicolumn{1}{c|}{}  & Title, \newline Title+one & Title, \newline Title+two & Title+one, \newline Title+two \\ 
      \hline
      Visual & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!5}p $<$ 0.05 \\ 
      \hline
      Textual & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & p = 0.352 \\ 
      \hline
      All \newline Participants & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 & \cellcolor{blue!15}p $<$ 0.01 \\ 
      \hline
    \end{tabular}
    \caption{Pairwise comparisons between preference groups for the 'fine-grained' ranking set (B). Exploratory analysis not included in pre-registration examined the differences in rankings overall, outside of the comparisons between groups.
    }
    \label{tab:rank_setB}
\end{table}

\subsection{RQ2: Semantic Levels and Takeaways}

RQ2 asks: How do the different semantic levels of text affect the type of information included in readers' takeaways? Further, when do readers include information in their takeaways that are not found either in the chart or the text? Which semantic levels of text do readers rely on when they form their takeaways? 

\pheading{Summary of Findings:} Through the following analyses, we found that participants' takeaways were influenced by \textit{some} semantic levels more than others. Specifically, annotations belonging to L3 and L4 had the greatest influence on the participants' takeaways, followed by L2. L1 annotations had almost no effect, in part because participants were very unlikely to provide any L1 takeaways. 

Overall, participants were most likely to provide L3 takeaways, synthesizing the information presented in an L2 or an L3 annotation. When provided with an L4 annotation in the chart, participants were more likely to include their own knowledge or experience, though they rarely did this. According to the self-reported question about reliance on text versus visual components of the chart, participants did not differ between semantic levels of text.



% \noindent
% \subsubsection{Qualitative Analysis}

\pheading{Details of Analysis:} Prior to investigating the hypotheses, two authors independently coded participant takeaways for the semantic level of the takeaway, whether the takeaway was a match to any of the provided annotations in the chart viewed, and whether the participant incorporated any information not contained in the chart and the text provided (e.g., a real-world event). In order to be considered a ``match'', the takeaway contained exact or similar language as used in the annotation provided. If a takeaway contained language belonging to more than one semantic level, the higher semantic level `trumped' the lower level and was assigned the higher level. This method follows the process used by Lundgard \& Satyanarayan \cite{lundgard2021accessible}.


Overall, inter-rater reliability was 0.818 (Kappa = 0.815 for takeaway level, Maxwell's RE = 0.727 for match, and Maxwell's RE = 0.912 for external information) \cite{gamer2012package}. A third author coded the conflicts and resolved all but four, which were discussed amongst the coders.

Overall, participants provided 736 takeaways. On average, each participant wrote 1.83 takeaways. Participants made 48 conclusions classified as L1, 132 classified as L2, 446 classified as L3, and 110 classified as L4. 245 of these takeaways (33.3\%) matched the annotations provided in the chart. Only 14 takeaways (1.9\%) included external information not already provided in the textual annotations. 



\subsubsection{H2a: Semantic Alignment between Text and Takeaways}

\textbf{H2a:} \textit{Reader takeaways will be more likely to contain a given semantic level if the text accompanying the chart also contains that semantic level. This will be true for all semantic levels.}

\smallskip
To examine 2a, we used logistic regression to analyze the relationship between the presence of different semantic levels of text on the chart and the semantic level of the reader's takeaway. We found \textbf{partial support} for this hypothesis.

First, we examined predicting factors for takeaways classified as L1. An example of an L1 takeaway is, ``\textit{The date range was 1960 to 2020}," (Participant 68). As mentioned previously, L1 takeaways were relatively uncommon. There were no significant influences on what semantic level of annotation may predict an L1 takeaway. So, H2a was not supported for L1.

Then, we examined predicting factors for L2 takeaways. An example of an L2 takeaway is, ``\textit{Immigration in 1982 was higher than in 1990}," (Participant 75). Participants were \textbf{1.6 times more likely} to provide an L2 takeaway when they were provided an L2 annotation than when they were shown an L1 annotation (95\% CI: [1.06, 2.40], p $<$ 0.05). They were also \textbf{2.0 times more likely} to provide an L2 takeaway with an L2 annotation than with a L3 annotation ([1.29, 2.95], p $<$ 0.01). However, they were \textbf{less likely }to provide an L2 takeaway after seeing a L4 annotation ([0.13, 0.24], p $<$ 0.01).
% so many numbers.... hopefully can push some of this to visual? tried ot use bolding to help make it more readable - not sure if it worked
Participants generally made takeaways containing L2 when they had viewed a chart which provided an L2 annotation, with the exception of charts which provided L4. They were more likely to make L2 takeaways when they saw L2 annotations, in comparison to when they saw annotations from L1 or L3. So, H2a was partially supported for L2.

L3 takeaways were the most frequently provided by participants overall. An example of an L3 takeaway is, `\textit{The national debt fell steeply in the early 90s before quickly rising to an all-time high}," (Participant 4). Participants were \textbf{2.2 times more likely} to provide an L3 takeaway when they were provided L3, in comparison to when they were provided L4 ([1.59, 3.05], p $<$ 0.01). Comparisons to other annotation levels did not affect the likelihood of making an L3 takeaway. 

Overall, participants provided mostly L3 takeaways, even in the presence of other levels. H2a is supported for L3, as the presence of an L3 annotation made it more likely that the participant would provide an L3 takeaway.

Finally, we examined L4 takeaways. An example of an L4 takeaway is, ``\textit{The tech boom in the early 1980s lead to a huge increase in median household incomes}," (Participant 215). Participants were significantly more likely to make L4 conclusions when they were provided with an L4 annotation: \textbf{6.1 times more likely} than when provided with L1 ([3.82, 10.19], p $<$ 0.01); \textbf{6.2 times more likely} than when provided with L2 ([3.85, 10.11], p $<$ 0.01); \textbf{3.2 times more likely} than when provided with L3 ([2.16, 4.79], p $<$ 0.01). 
Between all other semantic levels, L4 takeaways were most likely when the chart itself included L4 annotations. Therefore, H2a is supported for L4. 

\subsubsection{H2b: L1  Content and External Takeaways}

\textbf{H2b:} \textit{Readers will be more likely to include information in their takeaways that are not found in the visual information or text when L1 is present in the chart.}

\smallskip
To examine 2b, we used logistic regression to analyze the relationship between the presence of different semantic levels of text on the chart and the existence of external information in the participant's takeaway. This hypothesis was \textbf{not supported}. In fact, readers were more likely to include external information when L4 was present in the chart ([1.15, 72.73], p $<$ 0.05). However, there were very few takeaways which incorporated external information, as indicated by the extremely wide confidence interval. It remains unclear what kinds of annotations or  features may make readers more likely to include external information in their takeaways, but it is done infrequently.

\subsubsection{H2c, d, e: Preferences and Reliance on Visual vs. Text}

\noindent \textbf{H2c}: \textit{Readers will self-report a lower reliance on text when the text contains L1.}

\smallskip
\noindent \textbf{H2d}: \textit{Readers'  will self report takeaways relying more on text when the text contains L4.}

\smallskip
\noindent \textbf{H2e}: \textit{Readers with an overall preference for textual information will rely more on text within a chart.}

\smallskip
To examine hypotheses 2c-e, we performed a one-way ANOVA with post-hoc testing with Bonferroni correction. Reliance on textual and visual components of the chart was reported by participants on a 5-point Likert scale, where 1 indicated complete reliance on text and 5 indicated complete reliance on visual components. Participants were trained on what this language meant in the first section of the survey. 

Hypotheses 2c-d were \textbf{not supported}. Although there were differences between self-reported reliance on text between semantic levels ($F = 5.81$, $p = 0.016$, df = 1), follow-up pairwise testings with Bonferroni correction were not significant ($p > 0.05$). Average reliance ratings can be seen in Table \ref{tab:reliance_levels}. While takeaways relied more on text for L4 and less for L1, the difference was not large enough to make any claim as indicated in the above hypotheses.

%\vidya{wonder if Tables 4 and 5 can be formatted and placed differently. Right now they feel a bit orphaned in the paper.}

\begin{table}[h]
\def\arraystretch{1.5}
    \centering
    \begin{tabular}{ | m{0.24\linewidth} | m{0.13\linewidth} | m{0.13\linewidth} | m{0.13\linewidth} | m{0.13\linewidth} |} 
      \hline
        \textbf{Semantic Level} & L1 & L2 & L3 & L4 \\ 
      \hline
       \textbf{Avg. Reliance} & 3.84 & 3.76  & 3.65 & 3.60 \\ 
      \hline
    \end{tabular}
    \caption{Average reliance scores (1 = `entirely text', 5 = `entirely visual') between semantic levels displayed in the chart seen by participants.}
    \label{tab:reliance_levels}
\end{table}

% \noindent \textbf{H4d}: Readers with an overall preference for textual information will rely more on text within a chart. 

However, there was a difference between the \textsc{textual} and \textsc{visual} groups;  hypothesis H2e was \textbf{supported}. The \textsc{textual} group relied more on the text of a chart than the \textsc{visual} group, as shown in Table \ref{tab:reliance_pref}.

\begin{table}[h]
\def\arraystretch{1.5}
    \centering
    \begin{tabular}{ | m{0.3\linewidth} | m{0.12\linewidth} | m{0.12\linewidth} |} 
      \hline
        \textbf{Preference Group} & Textual & Visual \\ 
      \hline
       \textbf{Avg. Reliance} & 3.49 & 3.87 \\ 
      \hline
    \end{tabular}
    \caption{Average  reliance scores (1 = `entirely text', 5 = `entirely visual') between \textsc{textual} and \textsc{visual} groups (Bonferroni-adjusted p $<$ 0.01.)}
    \label{tab:reliance_pref}
\end{table}

\subsection{RQ3: Effect of Text Placement on Takeaways}

RQ3 asks: How does the placement of text affect how the reader integrates the text with the chart? 

\smallskip
\pheading{Summary of Findings:} Overall, the role of the placement of text varied between semantic levels. Participants were most likely  to match the L3 annotation provided when it was in the `title' position, but this effect was not true for any other level. For the other three levels, participants were more likely to match the annotation when the text was closer in proximity to the  itself. For L1, this meant being anchored to and describing one of the chart axes. For both L2 and L4, this meant being anchored to a specific point on the chart, accompanied by a visual annotation of the point. L3's content was usually broader, as it related to overall pattern syntheses, while L2's and L4's tended to be more specific and refer to single events or short spans.

\pheading{Details of Analysis:} The method for qualitatively coding the `position' of an annotation varied from that which was pre-registered. Each annotation was assigned a `role' during the stimuli creation stage, to ensure counterbalancing of the title position. For L1, other possible positions included `axis', with the annotation in a gray box next to the x- or y-axis, as well as `trend', for which the annotation was positioned in an unanchored callout box. For L2-L4, other positions also included `trend,' in which the the text was positioned next to an arrow or a gray band highlighting the relevant years. Additionally, these levels could have been positioned as a `point', which marked the point of interest with a dot matching the line in color. This coding system allowed us to better capture the role of `title' and compare its effect on the semantic level matched in participant takeaways.

To examine H3, we used logistic regression to analyze the relationship between the position or role of different semantic levels of text on the chart and the semantic level of the reader's takeaway. In this context, we examined only the takeaways which matched the annotations provided in the chart. We found partial support for this hypothesis.
\subsubsection{H3: Match of Takeaway to Semantic Level}
\noindent \textbf{H3}: Readers' takeaways will be most likely to match a given semantic level if the text containing that semantic level is positioned on as a title than in other aspects of the chart.

\smallskip
For takeaways which matched the L1 annotations, participants were most likely to match their takeaways to the annotation when it was positioned by an axis in the chart, rather than as a title. In fact, they were \textbf{11.3x more likely} to match the annotation when it was an axis than when it was a title ([3.18, 40.01], p $<$ 0.01), and \textbf{6.9 times more likely} than when it was a trend ([2.29, 20.80], p $<$ 0.01). So, this hypothesis was not supported for L1 takeaways. Titles were matched less often, while axes comments were matched most often.

Participants were most likely to match the L2 annotations when they were positioned as points, rather than titles. They were \textbf{2.0 times more likely} to match the annotation as a point than as a title ([1.00, 3.98], p $<$ 0.05). Thus, H3 was also not supported for L2 takeaways.

L3 takeaways, on the other hand, were most likely to be matched by participant takeaways when they were positioned as the title. They were \textbf{2.6 times more likely} to be matched when positioned as a title compared to positioned as a point ([1.52, 4.45]) and \textbf{2.0 times more likely} compared to positioning as a trend ([1.28, 3.33], p $<$ 0.01). H3 was supported for matched L3 annotations. 

In continuation of the overall trend, L4 takeaways were most likely to match when they were positioned as points, rather than as titles. Participants were \textbf{1.9 times more likely} to match the L4 annotation provided by the chart when it was positioned in the role of a point, compared to that of a title ([1.11, 3.22], p $<$ 0.05). 

==> original-submission/original04-discussion.tex <==
\section{Discussion}
\label{section:discussion}

This paper explores the effects of text progression and the various semantic levels on readers' preferences and takeaways. We discuss findings from our study and identify themes that support a better understanding of chart and text integration, along with practical implications for visualization tools and authoring practices. We use the notation $P\#$ when referring to participants in the discussion.

\subsection{Textual and visual preferences}
This work found significant differences in preferences between groups identified as preferring textual versus visual presentations of information. A non-trivial minority (14\%) of participants preferred a textual paragraph over a visual chart. Readers found the text easy to follow and understand. P15 stated, ``Like that it is easier to understand the changes in attendance when written out rather than the busy graph.'' Others found text to be a conducive medium for adding external information to support the data narrative - ``Like seeing the different points explained thoroughly and written in a story-like format [P41]'' and  ``I like that I get to learn details about why the President's approval rating grew and then dropped. Easy to read [P148].'' Others highlighted the distinction in preferences between \textsc{textual} and \textsc{visual} groups - ``I like this because it's very clear and gives me the information I need to know. I'm content with this. A more visual learner, however, would probably prefer the graph [P139].'' This feedback adds support to findings from prior work, which found a significant difference between text-only versus a text-plus-charts views, in a different setting (e.g., a chatbot showing simpler data in a bar chart format~\cite{hearst2019would} or natural language-generated data summary reports~\cite{ns}). These results underscore the importance for visualization research to consider the text-only case when comparing visualization options. 

On the flip side, the findings also showed that the most heavily annotated charts were preferred by those with strong visual preferences. P158 commented, ``I think all the extra facts and text on the chart are excellent ways to help people really know what's going on in the chart, and what factors play a role in how the data shapes up over time.'' P45 expressed that the representation was conducive for both \textsc{visual} and \textsc{textual} groups: ``I prefer the chart that combines both visual and written information the most. I think it helps the widest variety of learning styles to understand the chart.'' This result runs counter to concerns about the potential for such annotations to make the visual components of the chart appear cluttered.  Indeed, in their comments, many participants noted that they preferred the more heavily annotated charts despite the fact that they might appear more cluttered.

% quotes

% Like that it is easier to understand the changes in attendence when written out rather than the busy graph. - P15
% Straightforward. Just the text to focus on, and the text is organized in a way that is not distracting. - P27
% It's easy to read and understand this. I find it more intuitive to see and very simple. - P40
% Like seeing the different points explained thoroughly and written in a story-like format. - P41
% I like this because it's very clear and gives me the information I need to know. I'm content with this. A more visual learner, however, would probably prefer the graph. - P139
% It is very economical in the sense of there isn't much here to misinterpret. It just tells you the information. But, the information is conveyed in a low-effort fashion. - P191

% quote to support that text is a conducive medium for adding external information to support the narrative.
% I like that I get to learn details about why the President's approval rating grew and then dropped. Easy to read. - P148
% I like this more than the charts because it tries to give a fuller explanation to the data. - P263

% This method helps clearly and thoroughly explain the information, but it removes some of the shock value per se that a drastic drop and increase shows in a graphic rather than just text. - P172

\subsection{Over-texting was not penalized}
General guidelines for information sharing and presentation have shied away from adding too much text to imagery at the risk of overwhelming the viewer or not conforming to good design practices~\cite{tufte1985visual}. However, our study shows that the notion of over-texting was not penalized and was, in fact, often preferred. Readers liked the blend of text with charts, ranking charts annotated with more text higher than their sparser counterparts, including the text- and chart-only conditions. P10 indicated that, although they found the paragraph of text helpful, \textit{``the visuals of the graph + text allow me to more quickly assess the information.''} P31 called the combination \textit{``the best of both worlds.''}

%other possible useful quotes
%% "The chart summarizes the information in the narrative form in a way that is easier to digest, and is more impactful seeing it." - 49
%% While I understand things textually, having the visual really makes it stick in my mind. - 69
%% I like the charts over the text because it is easier for me to understand.  However, the text is better than the charts with incomplete information. - 99


Although heavily-annotated charts were generally preferred, the \textsc{textual} group ranked the text-only variant higher than the chart-only one, which we did not observe in the \textsc{visual} group. P178, who preferred the text-only variant, reported that they \textit{``like to read the words and use my own imagination for the imagery.''} P6 called the chart which displayed the same information as the text, \textit{``ugly to look at,''} a sentiment which was echoed by many who ranked that variant low. The text was \textit{``distracting''} and provided \textit{``too much information,''} .%cluttering the image. 

Similar to Lundgard \& Satyanarayan \cite{lundgard2021accessible}, some participants reported that their preference was influenced by their ability to draw their own conclusions about the data. While P261 appreciated the combination of context and \textit{``real information''}, P258 said \textit{``I like the raw data and being able to draw my own conclusions from the data. Data doesn't lie.''} about their preference for the textual version.

%other possible useful quotes
%%I don't like how convoluted the chart looks. I mean, it makes sense, but it's just a lot to take in. It's very busy. -36
%%This is way too busy and makes it hard to follow and see what I'm looking at. I feel it gives a lot of information but I feel it's too much work to take it in quickly. -151


\subsection{Text semantics influence reader takeaways }
 Authors often add text such as captions along with charts to provide additional context and previous work indicates the benefits of having both text and charts emphasize the same information to help with takeaways~\cite{kim2021towards}. However, we found that the semantic levels of text included with the chart can influence the kind of information that readers include in their takeaways. We observed that readers are not much influenced by L1-text and rather describe an overall pattern or shape in the chart, resulting in an L3 takeaway. We do however, see stronger influences of annotations from other semantic levels. For instance, in the presence of L2-text, many readers also include L2 statistical or relational comparisons about points in the line charts. Further, including external context to add to the narrative of the chart inspires readers to include that information in their own takeaways. 
 
 The topic of the chart and the external information associated with it, also influences the storytelling narrative that readers include. For example, we found that charts discussing data about presidential approval ratings and the immigration rates spurred takeaways that included the readers' own personal views and knowledge. 
 %P177 provided a takeaway which said, \textit{``There's no way a throwaway child hunger initiative in a country with overly redundant food welfare and a availability would shift almost half the country's opinion of him in a positive manner.''} They also followed this up with another response, writing \textit{``The President's rise and popularity had to have to do with something else's and the hunger initiative was just along for the ride so to speak.''} 
 For instance, P136  brought in external information, commenting, \emph{``The immigration numbers are likely undercounting the massive amount of illegials \emph{[sic]} that have entered the US in the last 40 years.''}



\subsection{Text placement matters}
Text provides the support and framing to charts for setting the context, clarify, and emphasize key insights in a chart. From our study, we found that the proximity of text to what it is describing in the chart, influences reader takeaways. For instance, readers included L1-text in their takeaways when the L1-text was describing one of the axes as an on-chart annotation. For example, P112 reported that their takeaway was, \textit{``showed years spanning from 1960 to 2010,''} after viewing a chart with the annotation \textit{``Years span 1960 to 2010, shown in decades.''} L2- and L4-text placed near a data point on the chart that they described, was more likely to be included in the takeaway as opposed to being positioned as the title of the chart. On the other hand, readers described overall trends from L3-text when it was placed as a title in the chart. These observations highlight an interesting interplay between spatial and text semantics in charts.

\subsection{Aesthetic preferences}
Beyond the utility of text with charts, readers had preferences as to the types of charts they liked, the design choices, and the placement of text in them. Many readers requested the use of color, improving the chart \textit{``by livening it up a bit''} (P31) or by making it \textit{``more eye catching''} (P112). However, not all readers agreed on the changes that should be made to the charts. A particularly contentious component was the use of gray arrows to highlight trends in the chart. 
Some readers appreciated these, saying, \textit{``I like the grey arrows shown next to text explaining why they are pointing in the direction they are''} (P19), or even requesting that an arrow be added to a chart which lacked it (P136). However, other participants said they \textit{``provide unnecessary visual clutter,''} and should instead \textit{``indicate the starting point of the events much like the dot represents the maximum and minimum points''} (P223). 

Another area of conflict between reader opinions was around the simplicity of the chart. Some enjoyed the simple nature of the visualization, while others told us to make it \textit{``more interesting (think Edward Tufte)''} (P28). Readers expressed opinions about the positioning or length of text, expressing strong dislike when the chart lacked a title, or when the title was too long: \textit{``used to pretty short and concise titles''} (135). 
%Others disliked when \textit{``the axis starts at 20k instead of 0''} (P196).

% another one for aesthetics in text
% I like that there are several facts present and I can understand why the number of immigrants moved as it did. I dislike that nothing is bolded, underlined, or otherwise emphasized. It is hard to tell what the speaker thinks is the most important part. - P289
%

%%%
%%%
% quote dump
%as far as what i dislike, the only thing i possibly would want to see is a little more color. for example, everything is printed in black numbers and letters. it might be better by livening it up a bit; perhaps use a different color for the dates or the heading.  anything to brighten things up a bit. - P31 (title+1)
% I like the grey arrows shown next to text explaining why they are pointing in the direction they are. - P19 (chart-story)
% I don't think the grey arrows are necessary because it's already easy to see the trend in the blue line.  I like the annotations as then I don't have to think as much about the visual. -P49 (chart-story)
%text should be a caption. More color differenatiation -P78 (title+1)
% I like that it's a fairly straight-forward graph.  It's a line graph that's easy to understand.  A possible dislike may be that it is rather simple.  It gets the job done, but doesn't give more detailed information. -P89 (no-text)
% The vertical axis lines are too light. P53 (title+1)
%Not really a dislike, but it would be nice if it used another color besides blue  to make it more eye catching. P112 (chart-story)
% I like the title, clearly labeled axes, and the additional text that explains the change in the graph pattern. I dislike that the scale is too wide. I would prefer narrower ticks in between the years and the trillions. - P134 (title+1)
%I think the title is pretty long, I am used to pretty short and concise titles.  - P135 (chart-story)
%I don't like that there isn't a title at the top of the graph. - P148 (no-text)
%I dislike that the axis starts at 20k instead of 0. P196 (title+1)
% I like it well enough. Might make the visual more interesting (think Edward Tufte).-P28 (chart-story)
%Good chart overall, a silver arrow alongside the cost-saving write up pointing down should have been added to the chart.  - P136 (chart-story)
%I think the arrows are a bit pointless and provide unnecessary visual clutter where they would be better situated if they were pointing vertically on the line to indicate the starting point of the events much like the dot represents the maximum and minimum points. P223 (chart-story)


%%%%%%%%%


% Takeaway Positions
% when people were matching L1s (mostly on axes)

% L3 -> title

% title, point, trend across all levels

% what should go in the title and what should go in the chart?
% L4 on the side

% L1 not a good title (chart takeaway paper)
% fact that people consistently used L3 from titles in their takeaways, guideleine to perhaps include L3-type title



%%%%%

==> original-submission/original05-futurework.tex <==
\section{Limitations and Future Work}
\label{section:lfw}

The results from our study highlight the importance of text with charts and how they together influence how readers glean insights from the data. They also point out that reader preferences
are also critical to take into consideration to determine the full experience and examine any impact of preference on comprehension. These observations provide both theoretical and practical implications for better understanding text in the larger context of visual analysis.

In this work, we explore the interplay between text and univariate line charts. Limiting some of the design options was key, as the combinatorial design space that accounts for the various semantic levels, amount, and placement of text, is rather large and complex to evaluate. We controlled for the amount of text in the charts by the presence or absence of one or more semantic levels of text in the chart. However, we need a more systematic way of assessing text progression, utilizing a more consistent computation of the amount of text and visual information in charts. Future work should explore how readers integrate text with other chart types, including dashboards and take into consideration other contexts such as mobile devices, print medium, and chatbot interfaces. 

We employed synthetically generated line charts to control for the experimental factors, but manually crafted the placement of annotations and embellishments such arrows with the guidance of a visualization expert. While this process provided some ecological validity, we would need to further explore other design parameters such as color to better understand their influence on readers' preferences and takeaways.

%how we computed textual vs visual -- need a good measure for this.
For our analysis, we used one part of a graphical literacy measure \cite{garcia2016measuring} that was correlated with preference, combining these responses with participants' self-reported behaviors around viewing charts and reading in long-form and in short. However, this may not provide clear or rigorous insight into the overall preference a reader has toward charts or text. Future work can develop and employ a more nuanced measure to capture and compare groups with different preferences.

As demonstrated from the results of this study, careful choices around semantic content in textual annotations, as well as the position of the annotation can influence what message or understanding the reader leaves the chart with after viewing. These results can also inform guidelines for supporting visual literacy by providing the reader with text which can help to scaffold their understanding of the information.



% hand-crafting of the stimuli (strength and a limitation); this was intended to add ecological validity

    % \item Further explore the placement of visual cues in the charts with text
    % \item Better captioning and annotation tools

% Only did univariate charts, no color, synthetic data -- can impact ecological validity


%Talk about guidelines for supporting visual literacy with the thoughtful use of text with charts...

==> original-submission/original06-conclusion.tex <==
\section{Conclusion}
\label{section:conclusions}

In this paper, we conducted a set of studies on nine examples of univariate line charts with varied amounts and types of annotations to better understand user preferences and takeaways from those charts. Findings from a study show that readers prefer a combination of textual and
visual communication over a single medium. They also indicate that the choice of semantic content and placement of the text in a chart can influence the readers’ takeaways. We propose guidelines to better design charts with text; using placement, visual cues and appropriate semantic levels, visual features in the chart can be better supported by their descriptions in the text. 

